Spectral Analysis and Preconditioned Iterative Solvers for Large Structured Linear Systems

In this thesis, the numerical solution of three different classes of problems have been studied. Specifically, new techniques have been proposed and their theoretical analysis has been performed, accompanied by a wide set of numerical experiments, for investigating further and comparing the effectiveness and performance of the presented approach. The first two belong to the research area of numerical linear algebra and concern the spectral analysis and preconditioning for Krylov subspace methods of the coefficient matrix of large structured linear systems. The third concerns a problem from the area of financial computing namely the pricing of an American put option.

==> REFERENCES.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Paris at 2022-04-30 19:27:42 +0300 


%% Saved with string encoding Unicode (UTF-8) 



@article{Ferrari2020,
	author = {Ferrari, P. and Barakitis, N. and Serra-Capizzano, S.},
	doi = {10.1002/nla.2332},
	journal = {Numer. Linear Algebra Appl.},
	number = {1},
	publisher = {Wiley},
	title = {Asymptotic spectra of large matrices coming from the symmetrization of {T}oeplitz structure functions and applications to preconditioning},
	url = {https://doi.org/10.1002/nla.2332},
	volume = {28},
	year = {2020},
	bdsk-url-1 = {https://doi.org/10.1002/nla.2332}}

@article{Magirou2020,
	author = {Magirou, E. and Vassalos, P. and Barakitis, N.},
	doi = {10.1016/j.cam.2019.112544},
	journal = {J. Comput. Appl. Math},
	pages = {112544},
	publisher = {Elsevier {BV}},
	title = {A policy iteration algorithm for the {A}merican put option and free boundary control problems},
	url = {https://doi.org/10.1016/j.cam.2019.112544},
	volume = {373},
	year = {2020},
	bdsk-url-1 = {https://doi.org/10.1016/j.cam.2019.112544}}

@article{Hon2018,
	author = {Hon, S. and Wathen, A.},
	fjournal = {Numerical Algorithms},
	issn = {1017-1398},
	journal = {Numer. Algorithms},
	mrclass = {65F08 (15A16 15B05 65F10 65F60)},
	mrnumber = {3878922},
	mrreviewer = {G\'{e}rard Meurant},
	number = {4},
	pages = {1211--1230},
	title = {Circulant preconditioners for analytic functions of {T}oeplitz matrices},
	volume = {79},
	year = {2018}}

@article{MR2609339,
	author = {Lee, S. T. and Pang, H. and Sun, H.},
	fjournal = {SIAM Journal on Scientific Computing},
	issn = {1064-8275},
	journal = {SIAM J. Sci. Comput.},
	mrclass = {65F60},
	mrnumber = {2609339},
	mrreviewer = {Jens-Peter M. Zemke},
	number = {2},
	pages = {774--792},
	title = {Shift-invert {A}rnoldi approximation to the {T}oeplitz matrix exponential},
	volume = {32},
	year = {2010}}

@article{MR2872597,
	author = {Lee, S. T. and Liu, X. and Sun, H.},
	fjournal = {Numerical Linear Algebra with Applications},
	issn = {1070-5325},
	journal = {Numer. Linear Algebra Appl.},
	mrclass = {65F60 (91G60)},
	mrnumber = {2872597},
	number = {1},
	pages = {87--101},
	title = {Fast exponential time integration scheme for option pricing with jumps},
	volume = {19},
	year = {2012}}

@article{FFHMS,
	author = {Ferrari, P. and Furci, I. and Hon, S. and Mursaleen, M. A. and Serra-Capizzano, S.},
	fjournal = {SIAM Journal on Matrix Analysis and Applications},
	issn = {0895-4798},
	journal = {SIAM J. Matrix Anal. Appl.},
	mrclass = {15B05 (15A18 65F08 65F15)},
	mrnumber = {4002720},
	number = {3},
	pages = {1066--1086},
	title = {The eigenvalue distribution of special 2-by-2 block matrix-sequences with applications to the case of symmetrized {T}oeplitz structures},
	volume = {40},
	year = {2019}}

@article{doi:10.1137/140974213,
	author = {Pestana, J. and Wathen, A.},
	fjournal = {SIAM Journal on Matrix Analysis and Applications},
	issn = {0895-4798},
	journal = {SIAM J. Matrix Anal. Appl.},
	mrclass = {65F08 (15B05 65F10)},
	mrnumber = {3323542},
	mrreviewer = {Ahmed Salam},
	number = {1},
	pages = {273--288},
	title = {A preconditioned {MINRES} method for nonsymmetric {T}oeplitz matrices},
	volume = {36},
	year = {2015}}

@book{MR890515,
	author = {U ~Grenander and G ~Szeg\H{o}},
	publisher = {Chelsea Publishing Co., New York, second edition},
	title = {{T}oeplitz forms and their applications},
	year = {1984}}

@article{MR952991,
	author = {Avram, F.},
	fjournal = {Probability Theory and Related Fields},
	issn = {0178-8051},
	journal = {Probab. Theory Related Fields},
	mrclass = {60F05 (60G15)},
	mrnumber = {952991},
	mrreviewer = {William P. McCormick},
	number = {1},
	pages = {37--45},
	title = {On bilinear forms in {G}aussian random variables and {T}oeplitz matrices},
	volume = {79},
	year = {1988}}

@article{MR851935,
	author = {Parter, S. V.},
	fjournal = {Linear Algebra and its Applications},
	issn = {0024-3795},
	journal = {Linear Algebra Appl.},
	mrclass = {47B35 (15A18)},
	mrnumber = {851935},
	mrreviewer = {A. B\"{o}ttcher},
	pages = {115--130},
	title = {On the distribution of the singular values of {T}oeplitz matrices},
	volume = {80},
	year = {1986}}

@article{Tyrtyshnikov19961,
	author = {Tyrtyshnikov, E. E.},
	fjournal = {Linear Algebra and its Applications},
	issn = {0024-3795},
	journal = {Linear Algebra Appl.},
	mrclass = {15A18 (15A57 47B35 65F15)},
	mrnumber = {1366576},
	mrreviewer = {A B\"{o}ttcher},
	pages = {1--43},
	title = {A unifying approach to some old and new theorems on distribution and clustering},
	volume = {232},
	year = {1996}}

@article{MR1258226,
	author = {Tyrtyshnikov, E. E.},
	fjournal = {Rossi\u{\i}skaya Akademiya Nauk. Doklady Akademii Nauk},
	issn = {0869-5652},
	journal = {Dokl. Akad. Nauk},
	mrclass = {47B35 (15A18 15A57 47A75 65F15)},
	mrnumber = {1258226},
	mrreviewer = {A. B\"{o}ttcher},
	number = {3},
	pages = {300--303},
	title = {New theorems on the distribution of eigenvalues and singular values of multilevel {T}oeplitz matrices},
	volume = {333},
	year = {1993}}

@article{SeTi,
	author = {Serra-Capizzano, S. and Tilli, P.},
	fjournal = {Journal of Inequalities and Applications},
	issn = {1025-5834},
	journal = {J. Inequal. Appl.},
	mrclass = {15A60 (15A45 47A30)},
	mrnumber = {1923734},
	mrreviewer = {Fabio Di Benedetto},
	number = {3},
	pages = {309--330},
	title = {On unitarily invariant norms of matrix-valued linear positive operators},
	volume = {7},
	year = {2002}}

@article{TyL1,
	author = {Tyrtyshnikov, E. E. and Zamarashkin, N. L.},
	fjournal = {Linear Algebra and its Applications},
	issn = {0024-3795},
	journal = {Linear Algebra Appl.},
	mrclass = {65F15 (15A18 42B05 47B35)},
	mrnumber = {1484073},
	mrreviewer = {A. Bultheel},
	pages = {15--27},
	title = {Spectra of multilevel {T}oeplitz matrices: advanced theory via simple matrix relationships},
	volume = {270},
	year = {1998}}

@article{MR1481397,
	author = {Zamarashkin, N. L. and Tyrtyshnikov, E. E.},
	fjournal = {Rossi\u{\i}skaya Akademiya Nauk. Matematicheski\u{\i} Sbornik},
	issn = {0368-8666},
	journal = {Mat. Sb.},
	mrclass = {47B35 (15A18 42A16 47A10)},
	mrnumber = {1481397},
	mrreviewer = {A B\"{o}ttcher},
	number = {8},
	pages = {83--92},
	title = {Distribution of the eigenvalues and singular numbers of {T}oeplitz matrices under weakened requirements on the generating function},
	volume = {188},
	year = {1997}}

@book{MR3674485,
	author = {Garoni, C. and Serra-Capizzano, S.},
	isbn = {978-3-319-53678-1; 978-3-319-53679-8},
	mrclass = {46-02 (15B05 46A45)},
	mrnumber = {3674485},
	mrreviewer = {Christopher P. Grant},
	pages = {xi+312},
	publisher = {Springer, Cham},
	title = {Generalized locally {T}oeplitz sequences: theory and applications. {V}ol. {I}},
	year = {2017}}

@article{NSV08,
	author = {Noutsos, D. and {Serra-Capizzano}, S. and Vassalos, P.},
	journal = {Linear Algebra Appl.},
	number = {2-3},
	pages = {600--624},
	publisher = {Elsevier {BV}},
	title = {The conditioning of {FD} matrix sequences coming from semi-elliptic differential equations},
	volume = {428},
	year = {2008}}

@article{V18,
	author = {Vassalos, P.},
	journal = {Electron. J. Linear Algebra},
	pages = {566--581},
	title = {Asymptotic results on the condition number of {FD} matrices approximating semi-elliptic {PDEs}},
	volume = {34},
	year = {2018}}

@book{MR3674485_vol2,
	author = {Garoni, C. and Serra-Capizzano, S.},
	publisher = {Springer, Cham},
	title = {Generalized locally {T}oeplitz sequences: theory and applications. {V}ol. {II}},
	year = {2018}}

@book{sauer_T,
	address = {USA},
	author = {Sauer, T.},
	edition = {2nd},
	isbn = {0321783670},
	publisher = {Addison-Wesley Publishing Company},
	title = {Numerical Analysis},
	year = {2011}}

@article{Meerschaert2004,
	author = {Meerschaert, M. and Tadjeran, C.},
	doi = {10.1016/j.cam.2004.01.033},
	journal = {J. Comput. Appl. Math.},
	number = {1},
	pages = {65--77},
	publisher = {Elsevier {BV}},
	title = {Finite difference approximations for fractional advection{\textendash}dispersion flow equations},
	url = {https://doi.org/10.1016/j.cam.2004.01.033},
	volume = {172},
	year = {2004},
	bdsk-url-1 = {https://doi.org/10.1016/j.cam.2004.01.033}}

@article{Meerschaert2006,
	author = {Meerschaert, M. and Tadjeran, C.},
	doi = {10.1016/j.apnum.2005.02.008},
	journal = {Appl. Numer. Math.},
	number = {1},
	pages = {80--90},
	publisher = {Elsevier {BV}},
	title = {Finite difference approximations for two-sided space-fractional partial differential equations},
	url = {https://doi.org/10.1016/j.apnum.2005.02.008},
	volume = {56},
	year = {2006},
	bdsk-url-1 = {https://doi.org/10.1016/j.apnum.2005.02.008}}

@article{Wang2010,
	author = {Wang, H. and Wang, K. and Sircar, T.},
	doi = {10.1016/j.jcp.2010.07.011},
	journal = {J. Comput. Phys.},
	number = {21},
	pages = {8095--8104},
	publisher = {Elsevier {BV}},
	title = {A direct $\mathcal{O}({N}\log^2{N})$ finite difference method for fractional diffusion equations},
	url = {https://doi.org/10.1016/j.jcp.2010.07.011},
	volume = {229},
	year = {2010},
	bdsk-url-1 = {https://doi.org/10.1016/j.jcp.2010.07.011}}

@article{donatelli161,
	author = {Donatelli, M. and Mazza, M. and Serra-Capizzano, S.},
	doi = {10.1016/j.jcp.2015.11.061},
	journal = {J. Comput. Phys.},
	pages = {262--279},
	publisher = {Elsevier {BV}},
	title = {Spectral analysis and structure preserving preconditioners for fractional diffusion equations},
	url = {https://doi.org/10.1016/j.jcp.2015.11.061},
	volume = {307},
	year = {2016},
	bdsk-url-1 = {https://doi.org/10.1016/j.jcp.2015.11.061}}

@article{moghaderi171,
	author = {Moghaderi, H. and Dehghan, M. and Donatelli, M. and Mazza, M.},
	doi = {10.1016/j.jcp.2017.08.064},
	journal = {J. Comput. Phys.},
	pages = {992--1011},
	publisher = {Elsevier {BV}},
	title = {Spectral analysis and multigrid preconditioners for two-dimensional space-fractional diffusion equations},
	url = {https://doi.org/10.1016/j.jcp.2017.08.064},
	volume = {350},
	year = {2017},
	bdsk-url-1 = {https://doi.org/10.1016/j.jcp.2017.08.064}}

@article{Tian2015,
	author = {Tian, W.Y. and Zhou, H. and Deng, W.},
	doi = {10.1090/s0025-5718-2015-02917-2},
	journal = {Math. Comput.},
	number = {294},
	pages = {1703--1727},
	publisher = {American Mathematical Society ({AMS})},
	title = {A class of second order difference approximations for solving space fractional diffusion equations},
	url = {https://doi.org/10.1090/s0025-5718-2015-02917-2},
	volume = {84},
	year = {2015},
	bdsk-url-1 = {https://doi.org/10.1090/s0025-5718-2015-02917-2}}

@article{axelsson861,
	author = {Axelsson, O. and Lindskog, G.},
	doi = {10.1007/bf01389448},
	journal = {Numer. Math.},
	number = {5},
	pages = {499--523},
	publisher = {Springer Nature},
	title = {On the rate of convergence of the preconditioned conjugate gradient method},
	url = {https://doi.org/10.1007/bf01389448},
	volume = {48},
	year = {1986},
	bdsk-url-1 = {https://doi.org/10.1007/bf01389448}}

@article{Tilli1998,
	author = {P. Tilli},
	doi = {10.1016/s0024-3795(97)10079-9},
	journal = {Linear Algebra Appl.},
	number = {1-3},
	pages = {91--120},
	publisher = {Elsevier {BV}},
	title = {Locally {T}oeplitz sequences: spectral properties and applications},
	url = {https://doi.org/10.1016/s0024-3795(97)10079-9},
	volume = {278},
	year = {1998},
	bdsk-url-1 = {https://doi.org/10.1016/s0024-3795(97)10079-9}}

@article{Taud2,
	author = {Serra-Capizzano, S.},
	journal = {Linear Algebra Appl.},
	pages = {37-78},
	title = {Spectral behavior of matrix sequences and discretized boundary value problems},
	volume = {337},
	year = {2001}}

@article{Capizzano2003,
	author = {Serra-Capizzano, S.},
	doi = {10.1016/s0024-3795(02)00504-9},
	journal = {Linear Algebra Appl.},
	pages = {371-402},
	publisher = {Elsevier {BV}},
	title = {Generalized locally {T}oeplitz sequences: spectral analysis and applications to discretized partial differential equations},
	url = {https://doi.org/10.1016/s0024-3795(02)00504-9},
	volume = {366},
	year = {2003},
	bdsk-url-1 = {https://doi.org/10.1016/s0024-3795(02)00504-9}}

@article{Estatico2008,
	author = {Estatico, C. and Serra-Capizzano, S.},
	doi = {10.1016/j.laa.2007.06.010},
	journal = {Linear Algebra Appl.},
	number = {2-3},
	pages = {564-585},
	publisher = {Elsevier {BV}},
	title = {Superoptimal approximation for unbounded symbols},
	url = {https://doi.org/10.1016/j.laa.2007.06.010},
	volume = {428},
	year = {2008},
	bdsk-url-1 = {https://doi.org/10.1016/j.laa.2007.06.010}}

@article{Skoro,
	author = {Serra-Capizzano, S.},
	doi = {10.1007/s002110050413},
	journal = {Numerische Mathematik},
	number = {1},
	pages = {117-142},
	publisher = {Springer Science and Business Media {LLC}},
	title = {A Korovkin-type theory for finite {T}oeplitz operators via matrix algebras},
	url = {https://doi.org/10.1007/s002110050413},
	volume = {82},
	year = {1999},
	bdsk-url-1 = {https://doi.org/10.1007/s002110050413}}

@article{Capizzano2000,
	author = {Serra-Capizzano, S.},
	doi = {10.1090/s0025-5718-00-01217-5},
	journal = {Mathematics of Computation},
	number = {232},
	pages = {1533-1559},
	publisher = {American Mathematical Society ({AMS})},
	title = {Korovkin tests, approximation, and ergodic theory},
	url = {https://doi.org/10.1090/s0025-5718-00-01217-5},
	volume = {69},
	year = {2000},
	bdsk-url-1 = {https://doi.org/10.1090/s0025-5718-00-01217-5}}

@article{glt-2,
	author = {Serra-Capizzano, S.},
	fjournal = {Linear Algebra Appl.},
	issn = {0024-3795},
	journal = {Linear Algebra Appl.},
	mrclass = {15A18 (47B35 65F10)},
	mrnumber = {2263117},
	mrreviewer = {A B\"{o}ttcher},
	number = {1},
	pages = {180--233},
	title = {The {GLT} class as a generalized {F}ourier analysis and applications},
	volume = {419},
	year = {2006}}

@article{Pang2012,
	author = {Pang, H. and Sun, H.},
	doi = {10.1016/j.jcp.2011.10.005},
	journal = {J. Comput. Phys.},
	number = {2},
	pages = {693--703},
	publisher = {Elsevier {BV}},
	title = {Multigrid method for fractional diffusion equations},
	url = {https://doi.org/10.1016/j.jcp.2011.10.005},
	volume = {231},
	year = {2012},
	bdsk-url-1 = {https://doi.org/10.1016/j.jcp.2011.10.005}}

@article{lei131,
	author = {Lei, S. and Sun, H.},
	doi = {10.1016/j.jcp.2013.02.025},
	journal = {J. Comput. Phys.},
	pages = {715--725},
	publisher = {Elsevier {BV}},
	title = {A circulant preconditioner for fractional diffusion equations},
	url = {https://doi.org/10.1016/j.jcp.2013.02.025},
	volume = {242},
	year = {2013},
	bdsk-url-1 = {https://doi.org/10.1016/j.jcp.2013.02.025}}

@article{noutsos161,
	author = {Noutsos, D. and Serra-Capizzano, S. and Vassalos, P.},
	doi = {10.1016/j.laa.2015.08.021},
	journal = {Linear Algebra Appl.},
	pages = {276--291},
	publisher = {Elsevier {BV}},
	title = {Essential spectral equivalence via multiple step preconditioning and applications to ill conditioned {T}oeplitz matrices},
	url = {https://doi.org/10.1016/j.laa.2015.08.021},
	volume = {491},
	year = {2016},
	bdsk-url-1 = {https://doi.org/10.1016/j.laa.2015.08.021}}

@article{NV-2008,
	author = {Noutsos, D. and Vassalos, P.},
	journal = {Comput. Math. with Appl.},
	number = {5},
	pages = {1255 - 1270},
	title = {Superlinear convergence for {PCG} using band plus algebra preconditioners for {T}oeplitz systems},
	volume = {56},
	year = {2008}}

@article{pang151,
	author = {Pang, H. and Hai-Wei Sun, H.},
	doi = {10.1007/s10915-015-0012-9},
	journal = {J. Sci. Comput.},
	number = {1},
	pages = {41--66},
	publisher = {Springer Nature},
	title = {Fast {N}umerical {C}ontour {I}ntegral {M}ethod for {F}ractional {D}iffusion {E}quations},
	url = {https://doi.org/10.1007/s10915-015-0012-9},
	volume = {66},
	year = {2015},
	bdsk-url-1 = {https://doi.org/10.1007/s10915-015-0012-9}}

@article{NSV_tcs,
	author = {Noutsos, D. and Serra-Capizzano, S. and Vassalos, P.},
	journal = {Theor. Comput. Sci},
	number = {2},
	pages = {557--579},
	title = {Matrix algebra preconditioners for multilevel {T}oeplitz systems do not insure optimal convergence rate},
	volume = {315},
	year = {2004}}

@inbook{NSV_con,
	address = {USA},
	author = {Noutsos, D. and Serra-Capizzano, S. and Vassalos, P.},
	isbn = {0821831771},
	pages = {313--322},
	publisher = {AMS},
	title = {Spectral Equivalence and Matrix Algebra Preconditioners for Multilevel {T}oeplitz Systems: A Negative Result.},
	year = {2001}}

@article{Lanczos1952,
	author = {C. Lanczos},
	doi = {10.6028/jres.049.006},
	journal = {J. Res. Natl. Bur. Stand.},
	number = {1},
	pages = {33},
	publisher = {National Institute of Standards and Technology ({NIST})},
	title = {Solution of systems of linear equations by minimized iterations},
	url = {https://doi.org/10.6028/jres.049.006},
	volume = {49},
	year = {1952},
	bdsk-url-1 = {https://doi.org/10.6028/jres.049.006}}

@article{Greenbaum1996,
	author = {Greenbaum, A. and Pt{\'{a}}k, V. and Strako{\v{s}}, Z.},
	doi = {10.1137/s0895479894275030},
	journal = {{SIAM} J Matrix Anal. Appl.},
	number = {3},
	pages = {465--469},
	publisher = {Society for Industrial {\&} Applied Mathematics ({SIAM})},
	title = {Any Nonincreasing Convergence Curve is Possible for {GMRES}},
	url = {https://doi.org/10.1137/s0895479894275030},
	volume = {17},
	year = {1996},
	bdsk-url-1 = {https://doi.org/10.1137/s0895479894275030}}

@book{Saad2003,
	author = {Y. Saad},
	doi = {10.1137/1.9780898718003},
	publisher = {Society for Industrial and Applied Mathematics},
	title = {Iterative Methods for Sparse Linear Systems},
	url = {https://doi.org/10.1137/1.9780898718003},
	year = {2003},
	bdsk-url-1 = {https://doi.org/10.1137/1.9780898718003}}

@article{Benzi2002,
	author = {M. Benzi},
	doi = {10.1006/jcph.2002.7176},
	journal = {J. Comput. Phys.},
	number = {2},
	pages = {418--477},
	publisher = {Elsevier {BV}},
	title = {Preconditioning Techniques for Large Linear Systems: A Survey},
	url = {https://doi.org/10.1006/jcph.2002.7176},
	volume = {182},
	year = {2002},
	bdsk-url-1 = {https://doi.org/10.1006/jcph.2002.7176}}

@article{mazza-pestana,
	author = {Mazza, M. and Pestana, J.},
	fjournal = {BIT. Numerical Mathematics},
	issn = {0006-3835},
	journal = {BIT},
	mrclass = {15B05 (15A18 65F08)},
	mrnumber = {3974049},
	number = {2},
	pages = {463--482},
	title = {Spectral properties of flipped {T}oeplitz matrices and related preconditioning},
	volume = {59},
	year = {2019}}

@article{HMS,
	author = {Hon, S. and Mursaleen, M. A. and Serra-Capizzano, S.},
	fjournal = {Linear Algebra Appl.},
	issn = {0024-3795},
	journal = {Linear Algebra Appl.},
	mrclass = {15B05 (65F15)},
	mrnumber = {3957457},
	pages = {32--50},
	title = {A note on the spectral distribution of symmetrized {T}oeplitz sequences},
	volume = {579},
	year = {2019}}

@article{Fasino2000,
	author = {Fasino, D. and Tilli, P.},
	doi = {10.1016/s0024-3795(99)00251-7},
	journal = {Linear Algebra Appl.},
	number = {1-3},
	pages = {155--163},
	publisher = {Elsevier {BV}},
	title = {Spectral clustering properties of block multilevel {H}ankel matrices},
	url = {https://doi.org/10.1016/s0024-3795(99)00251-7},
	volume = {306},
	year = {2000},
	bdsk-url-1 = {https://doi.org/10.1016/s0024-3795(99)00251-7}}

@article{Paige1975,
	author = {Paige, C. C. and Saunders, M. A.},
	doi = {10.1137/0712047},
	journal = {{SIAM} J. Numer. Anal.},
	number = {4},
	pages = {617--629},
	publisher = {Society for Industrial {\&} Applied Mathematics ({SIAM})},
	title = {Solution of Sparse Indefinite Systems of Linear Equations},
	url = {https://doi.org/10.1137/0712047},
	volume = {12},
	year = {1975},
	bdsk-url-1 = {https://doi.org/10.1137/0712047}}

@article{Saad1986,
	author = {Saad, Y. and Schultz, M. H.},
	doi = {10.1137/0907058},
	journal = {{SIAM} J. Sci. Comput.},
	number = {3},
	pages = {856--869},
	publisher = {Society for Industrial {\&} Applied Mathematics ({SIAM})},
	title = {{GMRES}: A Generalized Minimal Residual Algorithm for Solving Nonsymmetric Linear Systems},
	url = {https://doi.org/10.1137/0907058},
	volume = {7},
	year = {1986},
	bdsk-url-1 = {https://doi.org/10.1137/0907058}}

@inproceedings{reid1971method,
	author = {Reid, J. K.},
	booktitle = {Pro. the Oxford conference of institute of mathmatics and its applications},
	pages = {231--254},
	title = {On the method of conjugate gradients for the solution of large sparse systems of linear equations},
	year = {1971}}

@article{H.McK:65,
	author = {McKean, H.},
	journal = {Ind. Manag. Rev.},
	pages = {32--39},
	title = {A Free Boundary Problem for the Heat Equation Arising from a Problem in Mathematical Economics},
	volume = {6},
	year = {1965}}

@article{Jacka,
	author = {Jacka, S. D.},
	journal = {Math. Financ.},
	pages = {1--14},
	title = {Optimal Stopping and the \uppercase{A}merican Put},
	volume = {1},
	year = {1991}}

@article{CarrJarrowMyn,
	author = {Carr, P. and Jarrow, R. and Myneni, R.},
	journal = {Math. Financ.},
	pages = {87--106},
	title = {Alternative Characterizations of American Put Options},
	volume = {2},
	year = {1992}}

@article{Kim,
	author = {Kim, {I.J.}},
	journal = {Rev. Financial Stud.},
	pages = {547--572},
	title = {The Analytic Valuation of American Options},
	volume = {3},
	year = {1990}}

@article{Zhu18,
	author = {Zhu, {S. P.} and He, {X. J.} and Lu, {X. P.}},
	journal = {Quant. Finance},
	pages = {483--490},
	title = {A new integral equation formulation for \uppercase{A}merican put options},
	volume = {18},
	year = {2018}}

@article{J.Goo:02,
	author = {Goodman, J. and Ostrov, D.},
	journal = {SIAM J. Appl. Math.},
	pages = {1823--1835},
	title = {On the Early Exercise Boundary of the \uppercase{A}merican Put Option},
	volume = {62},
	year = {2002}}

@article{Barles,
	author = {Barles, G. and Burdeau, J. and Romano, K. and Samsoen, N.},
	journal = {Appl. Math. Finance},
	pages = {77--95},
	title = {Critical Stock price near expiration},
	volume = {5},
	year = {1995}}

@article{BrenSchw,
	author = {Brennan, M. and Schwartz, E.},
	journal = {J. Finance},
	pages = {449--462},
	title = {The Valuation of \uppercase{A}merican Put Options},
	volume = {32},
	year = {1977}}

@article{Scherer2011,
	author = {Scherer, R. and Kalla, S. L. and Tang, Y. and Huang, J.},
	doi = {10.1016/j.camwa.2011.03.054},
	journal = {Comput. Math. with Appl.},
	number = {3},
	pages = {902--917},
	publisher = {Elsevier {BV}},
	title = {The {G}r\"{u}nwald{\textendash}{L}etnikov method for fractional differential equations},
	url = {https://doi.org/10.1016/j.camwa.2011.03.054},
	volume = {62},
	year = {2011},
	bdsk-url-1 = {https://doi.org/10.1016/j.camwa.2011.03.054}}

@misc{Koh:14,
	author = {Kohn, R.},
	publisher = {Courant Institute of Mathematical Sciences},
	title = {Lecture notes in \uppercase{PDE'}s for \uppercase{F}inance},
	year = {2014}}

@book{Bellman,
	author = {Bellman, R.},
	publisher = {Princeton University Press},
	title = {Dynamic Programming},
	year = {1957}}

@book{Put:04,
	address = {New Jersey},
	author = {Puterman, M.},
	publisher = {John Wiley \& Sons, Inc.},
	title = {Markov \uppercase{D}ecision \uppercase{P}rocesses: \uppercase{D}iscrete \uppercase{S}tochastic \uppercase{D}ynamic \uppercase{P}rogramming},
	year = {2005}}

@article{E.Mag:77,
	author = {Mageirou, E.},
	journal = {J. Optim. Theory Appl.},
	pages = {51--61},
	title = {Iterative techniques for \uppercase{R}icatti game equations},
	volume = {22},
	year = {1977}}

@article{JackaVolat,
	author = {Maeda, J. and Jacka, S. D.},
	journal = {arXiv:1612.0078v1},
	title = {MARKET DRIVER VOLATILITY MODEL VIA POLICY IMPROVEMENT ALGORITHM},
	year = {2016}}

@article{BarErkVas,
	author = {Barakitis, N. and Ekstr{\"o}m, S.-E. and Vassalos, P.},
	journal = {Numer. Linear Algebra Appl.},
	title = {Preconditioners for Fractional Diffusion Equations Based on the Spectral Symbol},
	year = {(accepted)}}

@book{Hull,
	author = {Hull, J.},
	edition = {9th},
	publisher = {Pearson},
	title = {Options, Futures and Other Derivatives},
	year = {2017}}

@book{IsaacKell,
	author = {Isaacson, E. and Keller, H.},
	publisher = {Dover},
	title = {Analysis of Numerical Methods},
	year = {1994}}

@article{Tho70,
	author = {Kreiss, {H. O.} and Thom{\'e}e, V. and Widlund, O.},
	journal = {Comm. Pure Appl. Math.},
	pages = {241--259},
	title = {Smoothing of initial data and rates of convergence for parabolic difference equations},
	volume = {43},
	year = {1970}}

@article{Ran84,
	author = {Rannacher, R.},
	journal = {Numer. Math},
	pages = {309--327},
	title = {Finite element solution of diffusion problems with irregular data},
	volume = {43},
	year = {1984}}

@article{Forsyth1,
	author = {Forsyth, {P. A.} and Labahn, G.},
	journal = {J. Comput. Finance},
	pages = {1--44},
	title = {Numerical methods for controlled Hamilton-Jacobi Bellman PDEs in finance},
	volume = {11},
	year = {2007}}

@book{Elman2014,
	author = {Elman, H. and Silvester, D and Wathen, A.},
	doi = {10.1093/acprof:oso/9780199678792.001.0001},
	publisher = {Oxford University Press},
	title = {Finite Elements and Fast Iterative Solvers},
	url = {https://doi.org/10.1093/acprof:oso/9780199678792.001.0001},
	year = {2014},
	bdsk-url-1 = {https://doi.org/10.1093/acprof:oso/9780199678792.001.0001}}

@article{Pestana2019,
	author = {Pestana, J.},
	doi = {10.1137/18m1205406},
	journal = {{SIAM} Journal on Matrix Analysis and Applications},
	number = {3},
	pages = {870--887},
	publisher = {Society for Industrial {\&} Applied Mathematics ({SIAM})},
	title = {Preconditioners for Symmetrized {T}oeplitz and Multilevel {T}oeplitz Matrices},
	url = {https://doi.org/10.1137/18m1205406},
	volume = {40},
	year = {2019},
	bdsk-url-1 = {https://doi.org/10.1137/18m1205406}}

@book{Rynne2008,
	author = {Rynne, B. and Martin Youngson, M.},
	doi = {10.1007/978-1-84800-005-6},
	publisher = {Springer London},
	title = {Linear Functional Analysis},
	url = {https://doi.org/10.1007/978-1-84800-005-6},
	year = {2008},
	bdsk-url-1 = {https://doi.org/10.1007/978-1-84800-005-6}}

@article{JackaPI,
	author = {Jacka, {S. D.} and Mijatovic, A.},
	doi = {10.1080/17442508.2016.1187609},
	eprint = {https://doi.org/10.1080/17442508.2016.1187609},
	journal = {Stochastics},
	number = {1},
	pages = {348-359},
	publisher = {Taylor & Francis},
	title = {On the policy improvement algorithm in continuous time},
	url = {https://doi.org/10.1080/17442508.2016.1187609},
	volume = {89},
	year = {2017},
	bdsk-url-1 = {https://doi.org/10.1080/17442508.2016.1187609}}

@book{Wil91,
	author = {Williams, D.},
	publisher = {Cambridge University Press},
	title = {Probability with martingales},
	year = {1991}}

@article{magstef,
	author = {Magirou, E. and Vassalos, P.  and Barakitis, N.},
	journal = {arXiv preprint arXiv:2202.06418},
	title = {On a Boundary Updating Method for the Scalar {S}tefan Problem},
	year = {2022}}
	
@article{garoni2015,
  title={A general tool for determining the asymptotic spectral distribution of {H}ermitian matrix-sequences},
  author={Garoni, C. and {Serra-Capizzano}, S. and Vassalos, P.},
  journal={Operators and Matrices},
  volume={9},
  pages={549--561},
  year={2015}
}

@article{noutsos2006,
  title={Block band {T}oeplitz preconditioners derived from generating function approximations: analysis and applications},
  author={Noutsos, D. and Serra-Capizzano, S. and Vassalos, P.},
  journal={Numer. Math.},
  volume={104},
  number={3},
  pages={339--376},
  year={2006},
}

@article{noutsos2005,
  title={A preconditioning proposal for ill-conditioned {H}ermitian two-level {T}oeplitz systems},
  author={Noutsos, D. and {Serra-Capizzano}, S. and Vassalos, P.},
  journal={Numer. Linear Algebra Appl.},
  volume={12},
  number={2-3},
  pages={231--239},
  year={2005},
  }
  
  @article{NV2002,
  title={New band {T}oeplitz preconditioners for ill-conditioned symmetric positive definite {T}oeplitz systems},
  author={Noutsos, D. and Vassalos, P.},
  journal={SIMAX},
  volume={23},
  number={3},
  pages={728--743},
  year={2002},
  }
